Neuro-Symbolic Inductive Logic Programming with Logical Neural Networks

Recent work on neuro-symbolic inductive logic programming has led to promising approaches that can learn explanatory rules from noisy, real-world data. While some proposals approximate logical operators with differentiable operators from fuzzy or real-valued logic that are parameter-free thus diminishing their capacity to fit the data, other approaches are only loosely based on logic making it difficult to interpret the learned "rules". In this paper, we propose learning rules with the recently proposed logical neural networks (LNN). Compared to others, LNNs offer strong connection to classical Boolean logic thus allowing for precise interpretation of learned rules while harboring parameters that can be trained with gradient-based optimization to effectively fit the data. We extend LNNs to induce rules in first-order logic. Our experiments on standard benchmarking tasks confirm that LNN rules are highly interpretable and can achieve comparable or higher accuracy due to their flexible parameterization.

==> learn.tex <==
\begin{figure}
\begin{center}
\scriptsize
\begin{tikzpicture}[>=latex]
\node (mu_tilde) at (-0.45,1.1) [rectangle, draw, minimum height=1cm, minimum width=3mm,fill=green!20] {$\widehat{\mu}$};
\node (mu) at (0.55,1.1) [rectangle, draw, minimum height=1cm, minimum width=3mm] {$\mu$};
\node (gamma) at (0,0) [rectangle, draw, minimum height=1cm, minimum width=1.2cm,fill=red!20] {$\Gamma$};
\node (gen1) at (1.35,1.1) [rectangle, draw, minimum height=1cm, minimum width=3mm] {$\Gamma \mu$};
\draw[->] (mu_tilde) --  (mu) node[midway, above, align=center] {{\tt relu}};
\draw[->] (mu) --  (gen1);
\draw[->] (gamma) -- (1.35,0) -- (gen1);

\node (gen2) at (2.25,1.1) [rectangle, draw, minimum height=1cm, minimum width=3mm] {$\Upsilon \lambda$};
\node (nu) at (3.6,0) [rectangle, draw, minimum height=1cm, minimum width=1.2cm,,fill=red!20] {$\Upsilon$};
\draw[->] (nu) -- (2.25,0) -- (gen2);
\node (lambda_tilde) at (4.05,1.1) [rectangle, draw,fill=green!20, minimum height=1cm, minimum width=3mm] {$\widehat{\lambda}$};
\node (lambda) at (3.15,1.1) [rectangle, draw, minimum height=1cm, minimum width=3mm] {$\lambda$};
\draw[->] (lambda_tilde) -- (lambda) node[midway, above, align=center] {$\sigma$};
\draw[->] (lambda) -- (gen2);

\node (w) at (1.8,2.6) [rectangle, draw, minimum height=1cm, minimum width=3mm,draw,fill=lightgray!50] {$\rvw$};
\node (b) at (1.8,3.31) [rectangle, draw, minimum width=4mm,fill=lightgray!50] {$\beta$};
\node at (1.8,1.85) {+};
\draw[->] (gen1) -- (w);
\draw[->] (gen2) -- (w);

\node (x) at (4.05,2.6) [rectangle, draw, minimum height=1cm, minimum width=3mm,fill=yellow!50] {$\rvx$};

\node (dot) at (2.9,2.6) [circle,draw,minimum size=4mm,fill=blue!20]{};
\draw[->] (w) -- (dot);
\draw[->] (x) -- (dot);

\node at (2.9,2.25) {$\rvw^\top (1-\rvx)$};

\node (act) at (2.9,3.31) [circle,draw,minimum size=4mm,fill=blue!20]{};
\node at (3.3,3.31) {$-$};
\node (otpt) at (2.9,4) [circle,draw,minimum size=4mm,fill=blue!20]{};
\node at (3.6,4) {{\tt relu}-$1$};
\draw[->] (dot) -- (act);
\draw[->] (b) -- (act);
\draw[->] (act) -- (otpt);

\draw[draw=black,thick,dashed,rounded corners] (-0.7,-0.6) rectangle (4.3,1.7);

\end{tikzpicture}
\end{center}
\caption{Neural network for learning LNN-$\wedge$. Layers in the dashed box enforce constraints.}
\label{fig:andnn}
\end{figure}

\section{Learning Constrained Activations}
\label{sec:learn}

Enforcing inequality constraints is a challenge because constrained optimization with neural networks is a nascent field. While \citet{riegel:arxiv20} offer a specifically designed \emph{tailored} activation function that automatically satisfies the constraints described in the previous section, it limits LNN's applicability to various tasks such as ILP. In what follows, we present a more general approach that 1) learns LNN operators while adhering to the constraints, and 2) is applicable to \emph{any} formulation of LNNs as long as it involves \emph{linear} constraints. 

\citet{frerix:cvprw20} recently showed how to handle \emph{homogeneous} linear inequality constraints of the form $\mA \rvz \leq \vzero$ where $\mA$ denotes the coefficient matrix, and $\rvz$ denotes the parameters (in our case, $\beta$ and $\rvw$). We propose to extend \citeauthor{frerix:cvprw20}'s technique to handle constraints of the form $\mA \rvz \leq \rvb$, of which \myeqnref{eqn:constraints} is an instance, where $\rvb$ denotes the constants in the constraints. 

\par

We begin with the Minkowski-Weyl theorem:

\begin{theorem}
A set $\mathcal{C} = \{\rvz \, | \, \mA \rvz \leq \rvb\}$ is a convex polyhedron if and only if:
\begin{equation*}
\mathcal{C} = \left\{\Upsilon \mu + \Gamma \lambda \, \middle| \, \mu, \lambda \geq \vzero, \vone^\top \lambda = 1\right\}
\end{equation*}
where $\Upsilon$ and $\Gamma$ contain a finite number of rays and vertices, respectively.
\end{theorem}
which says that there exists a translation from $\mA, \rvb$ to $\Upsilon, \Gamma$ obtained via the \emph{double-description} method \citep{motzkin:tog53}. Assuming we can generate non-negative vectors $\mu, \lambda$ and additionally ensure that $\lambda$ sums to $1$, then one can access a point $\rvz = [\beta, \rvw]^\top$ from the feasible set $\mathcal{C}$ by computing $\Upsilon \mu + \Gamma \lambda$.

\myfigref{fig:andnn} depicts a \emph{neural network module} that can be included wherever we need to access $\beta, \rvw$ from the feasible set to implement LNN-$\wedge$. A similar module (with minor changes) exists that can be used to generate parameters for LNN-$\vee$. $\Gamma, \Upsilon$ (denoted in red) are used as weights for affine layers to transform $\mu, \lambda$ and summed together to generate $\beta, \rvw$ from the feasible set. To ensure that $\mu$ is non-negative and $\lambda$ adds to $1$, we generate these from auxilliary variables $\widehat{\mu}, \widehat{\lambda}$ using {\tt relu} \citep{nair:icml10} and $\sigma$ ({\tt softmax}), respectively:
\centerline{
\begin{minipage}{0.45\linewidth}
\begin{equation*}
\text{{\tt relu}}(\widehat{\mu}) = \max(0, \widehat{\mu})
\end{equation*}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\begin{equation*}
\sigma(\widehat{\lambda}) = e^{\widehat{\lambda}} / \vone^\top e^{\widehat{\lambda}}
\end{equation*}
\end{minipage}}

$\widehat{\lambda}, \widehat{\mu}$ (shown in green) form the real parameters that can be updated by propagating gradients using backpropagation during training while $\Gamma, \Upsilon$ are held constant. Once $\beta, \rvw$ are computed, the remaining operations needed for LNN-$\wedge$ are denoted using circular neurons (in blue) to combine with the input $\rvx$ (in yellow). The next section describes how to use LNN-$\wedge$ and LNN-$\vee$ modules for ILP.

